Second Order Accurate Hierarchical Approximate Factorization of Sparse SPD Matrices

We describe a second-order accurate approach to sparsifying the off-diagonal blocks in the hierarchical approximate factorizations of sparse symmetric positive definite matrices. The norm of the error made by the new approach depends quadratically, not linearly, on the error in the low-rank approximation of the given block. The analysis of the resulting two-level preconditioner shows that the preconditioner is second-order accurate as well. We incorporate the new approach into the recent Sparsified Nested Dissection algorithm [SIAM J. Matrix Anal. Appl., 41 (2020), pp. 715-746], and test it on a wide range of problems. The new approach halves the number of Conjugate Gradient iterations needed for convergence, with almost the same factorization complexity, improving the total runtimes of the algorithm. Our approach can be incorporated into other rank-structured methods for solving sparse linear systems.

==> abstract.tex <==
We describe an accurate approach to sparsifying the numerically low-rank matrix blocks in approximate hierarchical matrix factorizations.
The norm of the error made by the new approach depends quadratically on the error in the low-rank approximation of the given block.
We incorporate the new approach into Sparsified Nested Dissection, and test the new  algorithm on a wide range of symmetric positive definite systems.
 On all tested cases, the new approach results in at most half the number of Conjugate Gradient iterations needed for convergence, improving the total runtimes of the algorithm.
